IPO: Interpretable Prompt Optimization for Vision-Language Models

Pre-trained vision-language models like CLIP have remarkably adapted to various downstream tasks. Nonetheless, their performance heavily depends on the specificity of the input text prompts, which requires skillful prompt template engineering. Instead, current approaches to prompt optimization learn the prompts through gradient descent, where the prompts are treated as adjustable parameters. However, these methods tend to lead to overfitting of the base classes seen during training and produce prompts that are no longer understandable by humans. This paper introduces a simple but interpretable prompt optimizer (IPO), that utilizes large language models (LLMs) to generate textual prompts dynamically. We introduce a Prompt Optimization Prompt that not only guides LLMs in creating effective prompts but also stores past prompts with their performance metrics, providing rich in-context information. Additionally, we incorporate a large multimodal model (LMM) to condition on visual content by generating image descriptions, which enhance the interaction between textual and visual modalities. This allows for thae creation of dataset-specific prompts that improve generalization performance, while maintaining human comprehension. Extensive testing across 11 datasets reveals that IPO not only improves the accuracy of existing gradient-descent-based prompt learning methods but also considerably enhances the interpretability of the generated prompts. By leveraging the strengths of LLMs, our approach ensures that the prompts remain human-understandable, thereby facilitating better transparency and oversight for vision-language models.

==> Figures/app_metaprompt_figure.tex <==
\begin{figure}[t]
\textbf{INPUT}: \\
\noindent\fbox{
\parbox{\textwidth}{
\color{black}{
======================== Evaluating initial instructions =========================
}

\color{purple}{
You need to perform image classification on the large-scale visual recognition dataset based on visual features. Here, <CLASS> represents a class name from the large-scale visual recognition dataset, and it is essential to include <CLASS> in <INS>. 
\vspace{1em}

Below is the image description for each image:
}

\vspace{1em}
\color{blue}{
Image 0: The image showcases a plate of food featuring thinly sliced red meat, garnished with green herbs and possibly other spices or seasonings. 

Image 1: The image showcases a mouthwatering dish consisting of crispy grilled ribs with sticky sauce, accompanied by juicy apple slices on the side. 

\vspace{1em}

(… more image examples…)
\vspace{1em}
}

\color{purple}{
Below are some previous instructions with their scores. 
The scores consist of loss and accuracy. The loss value is equal to or greater than 0, while the accuracy varies from 0 to 100.
}

\color{darkpastelgreen}{
text:

a photo of a <CLASS>, a type of food.

scores:

loss: 0.78955078125, accuracy: 82.35294342041016



\vspace{1em}
(… more previous prompts and scores …)
\vspace{1em}

}

\color{purple}{
Generate an instruction different from all the instructions <INS> above, with a lower loss and higher accuracy than all the instructions <INS> above.  The instruction should begin with <INS> and end with </INS>. The instruction should be concise, effective, and generally applicable to all problems above.}

\color{black}{
================================= step 1 ================================
}

\color{purple}{
You need to perform image classification on the large-scale visual recognition dataset based on visual features. Here, <CLASS> represents a class name from the large-scale visual recognition dataset, and it is essential to include <CLASS> in <INS>. 
\vspace{1em}

Below is the image description for each image:
}

\vspace{1em}
\color{blue}{
Image 0: The image showcases a plate of food featuring thinly sliced red meat, garnished with green herbs and possibly other spices or seasonings. 

Image 1: The image showcases a mouthwatering dish consisting of crispy grilled ribs with sticky sauce, accompanied by juicy apple slices on the side. 

(… more image examples…)
\vspace{1em}
}\

\color{purple}{
Below are some previous instructions with their scores. 
The scores consist of loss and accuracy. The loss value is equal to or greater than 0, while the accuracy varies from 0 to 100.
}

\color{darkpastelgreen}{
text:

a photo of a <CLASS>, a type of food.

scores:

loss: 0.78955078125, accuracy: 82.35294342041016

\vspace{1em}

text:

Identify the <CLASS> in the image based on its unique visual features.

scores:

loss: 0.7109375, accuracy: 84.31372833251953

\vspace{1em}

text:

Inspect the image for key visual features of the <CLASS> and classify accordingly.

scores:

loss: 0.4912109375, accuracy: 85.35294342041016

\vspace{1em}
(… more previous prompts and scores …)
\vspace{1em}

}
\color{purple}{
Generate an instruction different from all the instructions <INS> above, with a lower loss and higher accuracy than all the instructions <INS> above.  The instruction should begin with <INS> and end with </INS>. The instruction should be concise, effective, and generally applicable to all problems above.}

}


}
\caption{Detailed of the input of our \ourprompt for prompt optimization on Food101~\cite{food101}.}
\label{fig:meta_prompt_detailed}
\end{figure}


==> Figures/app_moreoutputs.tex <==
\begin{figure}[t]
\textbf{OUTPUT}: \\
\noindent\fbox{
\parbox{\textwidth}{


\color{black}{
================================= step 1 ================================
}

\color{camel}{
(1)   <INS> Employ advanced visual recognition techniques to accurately classify the image featuring a <CLASS>. </INS>


\vspace{1em}
(2) <INS> Classify the image for <CLASS> identification based on detailed visual analysis.</INS>

\vspace{1em}
(3) <INS> Apply advanced pattern recognition techniques to classify the <CLASS> in the image with superior accuracy. </INS>

(4) <INS> Classify the image showcasing a <CLASS> with exceptional precision and minimal loss. </INS>

\vspace{1em}
(… more output prompts examples…)

\vspace{1em}

}


\color{black}{
================================= step 2 ================================
}

\color{camel}{
(1)   <INS> Utilize advanced visual analysis techniques to classify the <CLASS> in the image accurately. </INS>


\vspace{1em}
(2) <INS> Accurately classify the image of a <CLASS> based on its unique visual features. </INS>

\vspace{1em}
(3) <INS> Accurately classify the image featuring a <CLASS> with exceptional precision and minimal loss. </INS>

(4) <INS> Determine the visual attributes of the <CLASS> in the image for precise classification. </INS>

\vspace{1em}
(… more output prompts examples…)

\vspace{1em}

}

\color{black}{
================================= More steps  ================================
}

\vspace{1em}

\color{black}{
================================= step 99 ================================
}

\color{camel}{
(1)   <INS> Design a cutting-edge convolutional neural network for superior <CLASS> image classification accuracy and minimize loss. </INS>


\vspace{1em}
(2) <INS> Train an advanced convolutional neural network model for accurate and efficient <CLASS> image classification. </INS>

\vspace{1em}
(3) <INS> Identify the primary ingredient in the <CLASS> and describe its texture, color, and presentation. </INS>

(4) <INS> Develop a groundbreaking neural network model for accurate <CLASS> image classification with unprecedented precision and minimal loss. </INS>

\vspace{1em}
(… more output prompts examples…)

\vspace{1em}

}



\color{black}{
================================= step 100 ================================
}

\color{camel}{
(1)   <INS> Analyze the vibrant colors and unique petal structure of the <CLASS> food for precise classification. </INS>


\vspace{1em}
(2) <INS> Examine the vibrant colors and unique petal structure of the <CLASS> food for precise and accurate classification. </INS>

\vspace{1em}
(3) <INS> Identify the primary ingredient in the <CLASS> and describe its texture,
color, and presentation </INS>

(4) <INS> Enhance the classification of <CLASS> with cutting-edge deep learning models for optimal precision and minimal loss. </INS>

\vspace{1em}
(… more output prompts examples…)

\vspace{1em}

}


}


}
\caption{Detailed of the output of our \ourprompt for prompt optimization on Food101~\cite{food101}.}
\label{fig:meta_prompt_outputs}
\end{figure}

